Navigating Brain Language Representations: A Comparative Analysis of Neural Language Models and Psychologically Plausible Models

Neural language models, particularly large-scale ones, have been consistently proven to be most effective in predicting brain neural activity across a range of studies. However, previous research overlooked the comparison of these models with psychologically plausible ones. Moreover, evaluations were reliant on limited, single-modality, and English cognitive datasets. To address these questions, we conducted an analysis comparing encoding performance of various neural language models and psychologically plausible models. Our study utilized extensive multi-modal cognitive datasets, examining bilingual word and discourse levels. Surprisingly, our findings revealed that psychologically plausible models outperformed neural language models across diverse contexts, encompassing different modalities such as fMRI and eye-tracking, and spanning languages from English to Chinese. Among psychologically plausible models, the one incorporating embodied information emerged as particularly exceptional. This model demonstrated superior performance at both word and discourse levels, exhibiting robust prediction of brain activation across numerous regions in both English and Chinese.

==> tabs/interp.tex <==
\setlength{\tabcolsep}{1.5mm}
\begin{table*}[htbp]
	\centering
	\small
	\renewcommand\arraystretch{1}
	% \vspace{-0.4cm}
		% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \begin{tabular}{ccccccc|cccccc}
			\hline  
			\multirow{2}{*}{\textbf{Model}}&\multicolumn{6}{c|}{\textbf{LanguageLH}}&\multicolumn{6}{c}{\textbf{LanguageRH}}\\ 
			\cline{2-13}
			& Visi. & Moto. & Spac. & Time & Soci. & Emot. & Visi. & Moto. & Spac. & Time & Soci. & Emot.\\
			\hline
            \multicolumn{13}{c}{\textit{Natural Language Models}} \\
            \hline
			GloVe    &0.501&0.483&0.489&0.492&0.495&0.486&0.405&0.349&0.388&0.383&0.390&0.369 \\
			Word2Vec &0.524&0.494&0.522&0.516&0.531&0.541&0.424&0.354&0.412&0.420&0.418&0.418 \\
			BERT\textsubscript{\textnormal{base}} &0.570&0.567&0.567&0.556&0.597&0.601&0.467&0.441&0.456&0.477&0.494&0.483 \\
			GPT2\textsubscript{\textnormal{ori}} &0.573&0.585&0.545&0.595&0.591&0.613&0.473&0.460&0.437&0.511&0.484&0.502 \\
            BERT\textsubscript{\textnormal{lar}} &0.596&0.592&0.582&0.595&0.607&0.624&0.497&0.478&0.471&0.496&0.500&0.507 \\
            GPT2\textsubscript{\textnormal{med}} &0.573&0.585&0.545&0.595&0.591&0.613&0.472&0.460&0.436&0.511&0.484&0.502 \\
            \hline
            Mean  &0.556&0.551&0.542&0.558&0.569&0.579&0.456&0.424&0.433&0.466&0.462&0.463\\
            \hline
            \multicolumn{13}{c}{\textit{ Psychologically Plausible Models}} \\
            \hline
            LSM    &0.629&0.645&0.618&0.629&0.647&0.670&0.541&0.525&0.517&0.554&0.545&0.563 \\
            EBM    &0.645&0.667&0.641&0.657&0.666&0.685&0.567&0.564&0.548&0.580&0.576&0.595 \\
            NTM    &\textbf{0.665}&\textbf{0.686}&\textbf{0.660}&\textbf{0.669}&\textbf{0.692}&\textbf{0.714}&\textbf{0.589}&\textbf{0.583}&\textbf{0.576}&\textbf{0.587}&\textbf{0.603}&\textbf{0.624} \\
            \hline
            Mean &0.646&0.666&0.640&0.652&0.668&0.689&0.566&0.557&0.547&0.573&0.575&0.594 \\
			\hline 
    \end{tabular}
    \caption{Pearson correlation coefficient between predicted and true responses using PPMs and NLMs for six semantic features, including Vision, Motor, Space, Time, Social and Emotion.}
    \label{tab:interp}
     \vspace{-5mm}
\end{table*}

==> tabs/word.tex <==
\setlength{\tabcolsep}{1.5mm}
\begin{table*}[htbp]
	\centering
	\small
	\renewcommand\arraystretch{1}
	% \vspace{-0.4cm}
		% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \begin{tabular}{ccccccc|cccccc}
			\hline  
			\multirow{2}{*}{\textbf{Model}}&\multicolumn{6}{c|}{\textbf{English Sentence Paradigm}}&\multicolumn{6}{c}{\textbf{English Picture Paradigm}}\\ 
			\cline{2-13}
			& LaLH. & LaRH. & DMN & Body & Obje. & Visu. & LaLH. & LaRH. & DMN & Body & obje. & Visu.\\
			\hline
            \multicolumn{13}{c}{\textit{Neural Language Models}} \\
            \hline
			GloVe    &0.510&0.387&0.396&0.526&0.523&0.492&0.345&0.375&0.350&0.622&0.688&0.641 \\
			Word2Vec &0.546&0.429&0.441&0.567&0.566&0.533&0.384&0.409&0.394&0.655&0.722&0.679 \\
			BERT\textsubscript{\textnormal{base}} &0.595&0.485&0.487&0.615&0.613&0.587&0.432&0.459&0.453&0.698&0.760&0.721 \\
			GPT2\textsubscript{\textnormal{ori}} &0.613&0.508&0.512&0.629&0.631&0.602&0.448&0.481&0.465&0.705&0.763&0.728 \\
            BERT\textsubscript{\textnormal{lar}} &0.612&0.504&0.514&0.634&0.633&0.606&0.455&0.474&0.469&0.707&0.769&0.733 \\
            GPT2\textsubscript{\textnormal{med}} &0.613&0.508&0.512&0.629&0.632&0.602&0.447&0.481&0.464&0.705&0.763&0.728 \\
            \hline
            Mean  &0.582&0.470&0.477&0.600&0.600&0.570&0.418&0.447&0.432&0.682&0.744&0.705\\
            \hline
            \multicolumn{13}{c}{\textit{ Psychologically Plausible Models}} \\
            \hline
            LSM    &0.648&0.541&0.557&0.666&0.671&0.640&0.494&0.516&0.509&0.722&0.784&0.750 \\
            EBM    &0.679&0.583&0.597&0.702&0.703&0.676&0.542&0.558&0.550&\textbf{0.752}&\textbf{0.806}&\textbf{0.778} \\
            NTM    &\textbf{0.682}&\textbf{0.595}&\textbf{0.610}&\textbf{0.710}&\textbf{0.714}&\textbf{0.685}&\textbf{0.544}&\textbf{0.561}&\textbf{0.561}&0.740&0.796&0.767 \\
            \hline
            Mean &0.669&0.573&0.588&0.693&0.696&0.667&0.527&0.545&0.540&0.738&0.795&0.765 \\
			\hline 
    \end{tabular}
    \caption{Pearson correlation coefficients were computed for predicted and true values on word-level fMRI data using both NLMs and PPMs. We analyzed these correlations across three language-related regions (comprising LanguageLH (LaLH.), LanguageRH (LaRH.), and DMN) and three visual-related regions (including visual\_body (Body), visual\_object (Obje.), and visual networks (Visu.)).}
    \label{tab:word}
     \vspace{-5mm}
\end{table*}
